Adaptive Control of Unknown Pure Feedback Systems with Pure State Constraints

This paper deals with the tracking control problem for a class of unknown pure feedback system with pure state constraints on the state variables and unknown time-varying bounded disturbances. An adaptive controller is presented for such systems for the very first time. The controller is designed using the backstepping method. While designing it, Barrier Lyapunov Functions is used so that the state variables do not contravene its constraints. In order to cope with the unknown dynamics of the system, an online approximator is designed using a neural network with a novel adaptive law for its weight update. In the stability analysis of the system, the time derivative of Lyapunov function involves known virtual control coefficient with unknown direction and to deal with such problem Nussbaum gain is used to design the control law. Furthermore, to make the controller robust and computationally inexpensive, a novel disturbance observer is designed to estimate the disturbance along with neural network approximation error and the time derivative of virtual control input. The effectiveness of the proposed approach is demonstrated through a simulation study on the third-order nonlinear system.

==> bb <==
@article{Bechlioulis2014,
    title = {{A low-complexity global approximation-free control scheme with prescribed performance for unknown pure feedback systems}},
    year = {2014},
    journal = {Automatica},
    author = {Bechlioulis, Charalampos P. and Rovithakis, George A.},
    number = {4},
    pages = {1217--1226},
    volume = {50},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.automatica.2014.02.020},
    doi = {10.1016/j.automatica.2014.02.020},
    issn = {00051098},
    keywords = {Global approximation-free control, Low-complexity, Nonaffine systems, Prescribed performance, Uncertain systems}
}

@article{Ryan1991,
    title = {{A universal adaptive stabilizer for a class of nonlinear systems}},
    year = {1991},
    journal = {Systems and Control Letters},
    author = {Ryan, E. P.},
    number = {3},
    pages = {209--218},
    volume = {16},
    doi = {10.1016/0167-6911(91)90050-O},
    issn = {01676911},
    keywords = {Adaptive control, differential inclusions, discontinuous feedback, nonlinear system, universal stabilizers}
}

@article{Deng2017,
    title = {{Adaptive Control of Input Delayed Uncertain Nonlinear Systems with Time-Varying Output Constraints}},
    year = {2017},
    journal = {IEEE Access},
    author = {Deng, Wenxiang and Yao, Jianyong and Ma, Dawei},
    pages = {15271--15282},
    volume = {5},
    doi = {10.1109/ACCESS.2017.2730222},
    issn = {21693536},
    keywords = {Adaptive control, Lyapunov-Krasovskii functional, barrier function, input delay, output constraints, uncertainty}
}

@article{Meng2016,
    title = {{Adaptive neural control of a class of output-constrained nonaffine systems}},
    year = {2016},
    journal = {IEEE Transactions on Cybernetics},
    author = {Meng, Wenchao and Yang, Qinmin and Si, Jennie and Sun, Youxian},
    number = {1},
    pages = {85--95},
    volume = {46},
    doi = {10.1109/TCYB.2015.2394797},
    issn = {21682267},
    pmid = {25667363},
    keywords = {Adaptive control, Neural network (NN), Nonaffine systems, Output constraints, Transformation}
}

@article{Ziting2016,
    title = {{Adaptive Neural Control of Uncertain MIMO Nonlinear Systems With State and Input Constraints}},
    year = {2016},
    journal = {IEEE Transactions on Neural Networks and Learning Systems},
    author = {Ziting, Chen and Zhijun, Li and Philip, Chen C L},
    number = {99},
    pages = {1--13},
    volume = {PP},
    isbn = {9781509033645},
    doi = {10.1109/TNNLS.2016.2538779},
    issn = {21622388},
    keywords = {adaptive control, distubance observer, integral barrier lyapunov, rbf neural network, state feedback}
}

@article{He2015,
    title = {{Adaptive Neural Network Control of an Uncertain Robot With Full-State Constraints}},
    year = {2015},
    author = {He, Wei and Chen, Yuhao and Yin, Zhao and Member, Student},
    number = {3},
    pages = {1--10},
    volume = {46},
    doi = {10.1109/TCYB.2015.2411285},
    issn = {2168-2267}
}

@article{Ge1997,
    title = {{Adaptive neural network control of robot manipulators in task space}},
    year = {1997},
    journal = {IEEE Transactions on Industrial Electronics},
    author = {Ge, Shuzhi S. and Hang, C. C. and Woon, L. C.},
    number = {6},
    pages = {746--752},
    volume = {44},
    doi = {10.1109/41.649934},
    issn = {02780046},
    keywords = {Adaptive control, Neural network, Robot manipulator, Task space}
}

@article{Xudong1998,
    title = {{Adaptive nonlinear design without a priori knowledge of control directions}},
    year = {1998},
    journal = {IEEE Transactions on Automatic Control},
    author = {Xudong, Ye and Jingping, Jiang},
    number = {11},
    pages = {1617--1621},
    volume = {43},
    doi = {10.1109/9.728882},
    issn = {00189286},
    keywords = {Adaptive control, Nonlinear, Uncertain systems}
}

@article{Liu2017,
    title = {{Automatica Barrier Lyapunov functions for Nussbaum gain adaptive control of full state constrained nonlinear systems ✩}},
    year = {2017},
    journal = {Automatica},
    author = {Liu, Yan-jun and Tong, Shaocheng},
    pages = {143--152},
    volume = {76},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.automatica.2016.10.011},
    doi = {10.1016/j.automatica.2016.10.011},
    issn = {0005-1098},
    keywords = {barrier lyapunov functions, full state constraints, nussbaum gain control}
}

@article{Zajkowska2011,
    title = {{F ( t ) S ( t )}},
    year = {2011},
    author = {Zajkowska, Agata and Ski, Łukasz Derpe Ń and Seweryn, Andrzej},
    number = {1},
    pages = {137--142},
    volume = {5},
    isbn = {9781424467464},
    arxivId = {arXiv:1611.02567v1},
    keywords = {http://dx.doi.org/10.1029/JB082i005p00803, doi:10.}
}

@article{Tee2009,
    title = {{Output-feedback adaptive control of electrostatic microactuators}},
    year = {2009},
    journal = {Proceedings of the American Control Conference},
    author = {Tee, Keng Peng and Ge, Shuzhi Sam and Tay, Eng Hock},
    number = {2},
    pages = {4215--4220},
    volume = {17},
    isbn = {9781424445240},
    doi = {10.1109/ACC.2009.5160213},
    issn = {07431619}
}

@article{Nussbaum1983,
    title = {{Some remarks on a conjecture in parameter adaptive control}},
    year = {1983},
    journal = {Systems and Control Letters},
    author = {Nussbaum, Roger D.},
    number = {5},
    pages = {243--246},
    volume = {3},
    doi = {10.1016/0167-6911(83)90021-X},
    issn = {01676911},
    keywords = {Parameter adaptive control}
}

@article{Tang2013,
    title = {{Tangent barrier Lyapunov functions for the control of output-constrained nonlinear systems}},
    year = {2013},
    journal = {IFAC Proceedings Volumes (IFAC-PapersOnline)},
    author = {Tang, Zhong Liang and Tee, Keng Peng and He, Wei},
    number = {PART 1},
    pages = {449--455},
    volume = {3},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.automatica.2008.11.017},
    isbn = {9783902823458},
    doi = {10.3182/20130902-3-CN-3020.00122},
    issn = {14746670},
    keywords = {Backstepping design, Output constraints, Tangent barrier lyapunov functions}
}

@article{Skafidas1999=Ir,
    title = {{= Ir}},
    year = {1999},
    author = {Skafidas, E and Mareels, I M Y and Evans, R J},
    number = {4},
    pages = {868--872},
    volume = {44}
}

@article{Zhang2006A,
    title = {{A global Implicit Function Theorem without initial point and its applications to control of non-affine systems of high dimensions ✩}},
    year = {2006},
    author = {Zhang, Weinian and Ge, Shuzhi Sam},
    pages = {251--261},
    volume = {313},
    doi = {10.1016/j.jmaa.2005.08.072},
    keywords = {global existence, implicit function, state feedback control}
}

@article{Chen2014AEchniques,
    title = {{A N onlinear E xact D isturbance O bserver I nspired by S liding M ode T echniques}},
    year = {2014},
    author = {Chen, Xinkai},
    pages = {181--185},
    volume = {1},
    isbn = {9781479963812},
    keywords = {adaptive method, disturbance observer, sliding mode}
}

@article{Khalil2014ADerivative,
    title = {{A new definition of fractional derivative}},
    year = {2014},
    journal = {Journal of Computational and Applied Mathematics},
    author = {Khalil, R. and Al Horani, M. and Yousef, A. and Sababheh, M.},
    pages = {65--70},
    volume = {264},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.cam.2014.01.002},
    isbn = {0370-1573},
    doi = {10.1016/j.cam.2014.01.002},
    issn = {03770427},
    pmid = {27063839},
    arxivId = {cond-mat/9402042},
    keywords = {Fractional derivative, Fractional integral}
}

@article{Lu2015AStability,
    title = {{A note on finite-time and fixed-time stability}},
    year = {2015},
    author = {Lu, Wenlian and Liu, Xiwei and Chen, Tianping},
    pages = {1--13},
    url = {http://arxiv.org/abs/1507.07160},
    doi = {10.1016/j.neunet.2016.04.011},
    issn = {08936080},
    pmid = {27239892},
    arxivId = {1507.07160},
    keywords = {consensus, event-triggered algorithm, time-varying topology}
}

@article{Yang2007AdaptiveNetworks,
    title = {{Adaptive Control of a Class of Nonaffine Systems Using Neural Networks}},
    year = {2007},
    journal = {IEEE Trans. Neural Netw.},
    author = {Yang, B.- J and Calise, A J},
    number = {4},
    pages = {1149--1159},
    volume = {18}
}

@article{Zou2008AdaptiveApproach,
    title = {{Adaptive Control of a Class of Nonlinear Pure-Feedback Systems Using Fuzzy Backstepping Approach}},
    year = {2008},
    journal = {Fuzzy Systems, IEEE Transactions on},
    author = {Zou, An-Min and Hou, Zeng-Guang and Tan, Min},
    number = {4},
    pages = {886--897},
    volume = {16},
    isbn = {1063-6706 VO - 16},
    doi = {10.1109/TFUZZ.2008.917301},
    keywords = {Adaptive, Adaptive control, Approximation error, Backstepping, Control systems, Fuzzy control, Fuzzy logic, Fuzzy systems, Nonlinear control systems, Nonlinear dynamical systems, Robust control, adaptive control, algebra, algebraic loop problems, approximation errors, approximation theory, backstepping control, closed loop systems, closed-loop system, compensation, feedback, filtering theory, fuzzy control, fuzzy logic, fuzzy logic systems, nonlinear control systems, nonlinear pure-feedback systems, nonlinear strict-feedback systems, nonlinear systems, pure-feedback form, robust control, robust fuzzy backstepping control, signal filtering, single-input-single-output nonlinear systems, smooth robust compensators, unknown plant dynamics}
}

@article{Esfandiari2014AdaptiveNetworks,
    title = {{Adaptive Control of Uncertain Nonaffine Nonlinear Systems With Input Saturation Using Neural Networks}},
    year = {2014},
    journal = {Neural Networks and Learning Systems, IEEE Transactions on},
    author = {Esfandiari, Kasra and Member, Student and Abdollahi, Farzaneh and Member, Senior and Talebi, Heidar Ali},
    number = {10},
    pages = {1--12},
    volume = {26},
    doi = {10.1109/TNNLS.2014.2378991},
    issn = {2162-237X}
}

@article{Liu2017AdaptiveSystems,
    title = {{Adaptive controller design-based ABLF for a class of nonlinear time-varying state constraint systems}},
    year = {2017},
    journal = {IEEE Transactions on Systems, Man, and Cybernetics: Systems},
    author = {Liu, Yan Jun and Lu, Shumin and Li, Dongjuan and Tong, Shaocheng},
    number = {7},
    pages = {1546--1553},
    volume = {47},
    doi = {10.1109/TSMC.2016.2633007},
    issn = {21682232},
    keywords = {Adaptive control, Full state constraints, Nonlinear systems, Uncertain systems}
}

@article{Dhar2017AdaptiveSystem,
    title = {{Adaptive Critic based Event-Triggered Control for HVAC System}},
    year = {2017},
    journal = {IEEE Transactions on Industrial Informatics},
    author = {Dhar, Narendra Kumar and Verma, Nishchal Kumar and Behera, Laxmidhar},
    number = {1},
    pages = {178--188},
    volume = {14},
    doi = {10.1109/TII.2017.2725899},
    issn = {15513203},
    keywords = {Adaptive systems, Discrete-time systems, HVAC system, Nonlinear dynamical systems, Real-time systems, Trajectory, adaptive critic control, discrete time system, event-triggered controller, stability}
}

@article{Wen2011AdaptiveSystems,
    title = {{Adaptive fuzzy controller for a class of strict-feedback nonaffine nonlinear systems}},
    year = {2011},
    journal = {Journal of Systems Engineering and Electronics},
    author = {Wen, Jie and Jiang, Changsheng},
    number = {6},
    pages = {967--974},
    volume = {22},
    url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=6133377},
    doi = {10.3969/j.issn.1004-4132.2011.06.013},
    issn = {1004-4132},
    keywords = {backstepping ap-, fuzzy control, nonaf fi ne system}
}

@article{Li2014AdaptiveApproach,
    title = {{Adaptive Fuzzy Robust Output Feedback Control of Nonlinear Systems With Unknown Dead Zones Based on a Small-Gain Approach}},
    year = {2014},
    journal = {IEEE Transactions on Fuzzy Systems},
    author = {Li, Y. and Tong, S. and Liu, Y. and Li, T.},
    number = {1},
    pages = {164--176},
    volume = {22},
    url = {http://ieeexplore.ieee.org/ielx7/91/6729075/06471803.pdf?tp=&arnumber=6471803&isnumber=6729075%5Cnhttp://ieeexplore.ieee.org/xpl/articleDetails.jsp?arnumber=6471803&sortType%3Dasc_p_Sequence%26filter%3DAND%28p_IS_Number%3A6729075%29},
    isbn = {1063-6706{\textbackslash}r1941-0034},
    doi = {10.1109/TFUZZ.2013.2249585},
    issn = {1063-6706}
}

@article{Tang2010AdaptiveFunction,
    title = {{Adaptive Neural Control for Output Feedback Nonlinear Systems Using a Barrier Lyapunov Function}},
    year = {2010},
    journal = {Ieee Transactions on Neural Networks},
    author = {Tang, Zhong Liang and Tee, Keng Peng and He, Wei},
    number = {8},
    pages = {1339--1345},
    volume = {21},
    url = {http://arc.aiaa.org/doi/10.2514/6.2016-1865%0Ahttp://dx.doi.org/10.3182/20130902-3-CN-3020.00168%0Ahttp://dx.doi.org/10.1016/j.automatica.2011.08.044%0Ahttp://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=5499019%0Ahttp://arc.aiaa.org/doi/abs/10.2514/6.20},
    isbn = {9783902823458},
    doi = {10.3182/20130902-3-CN-3020.00122},
    issn = {14746670},
    keywords = {Backstepping design, Output constraints, Tangent barrier lyapunov functions}
}

@article{Yang2015AdaptiveNonlinearities,
    title = {{Adaptive Neural Control of Nonaffine Systems with Unknown Control Coefficient and Nonsmooth Actuator Nonlinearities}},
    year = {2015},
    journal = {IEEE Transactions on Neural Networks and Learning Systems},
    author = {Yang, Zaiyue and Yang, Qinmin and Sun, Youxian},
    number = {8},
    pages = {1822--1827},
    volume = {26},
    doi = {10.1109/TNNLS.2014.2354533},
    issn = {21622388},
    pmid = {25265633},
    keywords = {Adaptive neural control, nonaffine systems, nonsmooth nonlinearity, unknown control coefficient}
}

@article{Meng2015AdaptiveConstraints,
    title = {{Adaptive neural control of nonlinear MIMO systems with time-varying output constraints}},
    year = {2015},
    journal = {IEEE Transactions on Neural Networks and Learning Systems},
    author = {Meng, Wenchao and Yang, Qinmin and Sun, Youxian},
    number = {5},
    pages = {1074--1085},
    volume = {26},
    publisher = {IEEE},
    doi = {10.1109/TNNLS.2014.2333878},
    issn = {21622388},
    pmid = {25051562},
    keywords = {Adaptive control, constraints, neural network (NN), nonlinear multiple-input multiple-output (MIMO) sy, time-varying system.}
}

@article{Ge2004AdaptiveCoefficients.,
    title = {{Adaptive neural control of nonlinear time-delay systems with unknown virtual control coefficients.}},
    year = {2004},
    journal = {IEEE transactions on systems, man, and cybernetics. Part B, Cybernetics : a publication of the IEEE Systems, Man, and Cybernetics Society},
    author = {Ge, Shuzhi Sam and Hong, Fan and Lee, Tong Heng},
    number = {1},
    pages = {499--516},
    volume = {34},
    issn = {1083-4419},
    pmid = {15369088}
}

@article{Ge2004AdaptiveSystems,
    title = {{Adaptive neural control of uncertain MIMO nonlinear systems}},
    year = {2004},
    journal = {IEEE Transactions on Neural Networks},
    author = {Ge, Shuzhi Sam and Wang, Cong},
    number = {3},
    pages = {674--692},
    volume = {15},
    isbn = {1045-9227 VO - 15},
    doi = {10.1109/TNN.2004.826130},
    issn = {10459227},
    pmid = {15384555},
    keywords = {Adaptive neural control, Backstepping, Block-triangular form, Multi-input/multi-output (MIMO) nonlinear systems, Neural networks (NN)}
}

@article{He2017AdaptiveFunction,
    title = {{Adaptive Neural Network Control of a Marine Vessel with Constraints Using the Asymmetric Barrier Lyapunov Function}},
    year = {2017},
    journal = {IEEE Transactions on Cybernetics},
    author = {He, Wei and Yin, Zhao and Sun, Changyin},
    number = {7},
    pages = {1641--1651},
    volume = {47},
    isbn = {9783902823458},
    doi = {10.1109/TCYB.2016.2554621},
    issn = {21682267},
    keywords = {Adaptive control, barrier Lyapunov function, constraints, marine vessel, neural networks (NNs), trajectory tracking}
}

@article{Zhang2009AdaptiveDirections,
    title = {{Adaptive neural network tracking control of MIMO nonlinear systems with unknown dead zones and control directions}},
    year = {2009},
    journal = {IEEE Transactions on Neural Networks},
    author = {Zhang, Tianping and Ge, Shuzhi S.},
    number = {3},
    pages = {483--497},
    volume = {20},
    doi = {10.1109/TNN.2008.2010349},
    issn = {10459227},
    pmid = {19193510},
    keywords = {Adaptive control, Dead zone, Neural network (NN) control, Nussbaum function, Sliding mode control}
}

@article{Systems2016AdaptiveNonlinear,
    title = {{Adaptive Neural Network-Based Event-Triggered Control of Single-Input Single-Output Nonlinear}},
    year = {2016},
    author = {Systems, Discrete-time and Sahoo, Avimanyu and Xu, Hao and Jagannathan, Sarangapani and Member, Senior},
    number = {1},
    pages = {151--164},
    volume = {27}
}

@article{Zhao2018AdaptiveSaturation,
    title = {{Adaptive NN finite-time tracking control of output constrained nonlinear system with input saturation}},
    year = {2018},
    journal = {Nonlinear Dynamics},
    author = {Zhao, Shiyi and Liang, Hongjing and Du, Peihao and Qi, Suwen},
    number = {4},
    pages = {1845--1856},
    volume = {92},
    publisher = {Springer Netherlands},
    url = {https://doi.org/10.1007/s11071-018-4167-4},
    doi = {10.1007/s11071-018-4167-4},
    issn = {1573269X},
    keywords = {Barrier Lyapunov functions (BLFs), Finite-time control, Input saturation, Neural networks (NNs), Output constraints}
}

@article{Li2011AdaptiveSystems,
    title = {{Adaptive NN tracking control of nonlinear discrete-time systems}},
    year = {2011},
    journal = {The Fourth International Workshop on Advanced Computational Intelligence},
    author = {Li, DongJuan and Cui, Yang and Liu, YanJun},
    number = {3},
    pages = {133--137},
    volume = {45},
    isbn = {978-1-61284-373-5},
    doi = {10.1109/IWACI.2011.6159989}
}

@book{Liu2011AdvancedSystems,
    title = {{Advanced Sliding Mode Control for Mechanical Systems}},
    year = {2011},
    author = {Liu, Jinkun and Wang, Xinhua},
    pages = {356},
    url = {http://link.springer.com/10.1007/978-3-642-20907-9},
    isbn = {978-3-642-20906-2},
    doi = {10.1007/978-3-642-20907-9}
}

@book{CorkeALGORITHMS,
    title = {{ALGORITHMS}},
    author = {Corke, Peter},
    isbn = {9783319544120}
}

@article{Jin2017AnDisturbances,
    title = {{An Adaptive Control Architecture for Cyber-Physical System Security in the Face of Sensor and Actuator Attacks and Exogenous Stochastic Disturbances}},
    year = {2017},
    author = {Jin, Xu and Haddad, Wassim M and Hayakawa, Tomohisa},
    number = {Cdc},
    pages = {1380--1385},
    volume = {62},
    isbn = {9781509028726}
}

@article{Tabuada2012AnControl,
    title = {{An Introduction to Event-triggered and Self-triggered Control}},
    year = {2012},
    author = {Tabuada, P},
    pages = {3270--3285},
    isbn = {9781467320665},
    keywords = {Control over communications, Networked control systems}
}

@article{Li2017Approximation-BasedConstraints,
    title = {{Approximation-Based Adaptive Neural Tracking Control of Nonlinear MIMO Unknown Time-Varying Delay Systems With Full State Constraints}},
    year = {2017},
    author = {Li, Da-peng and Li, Dong-juan and Liu, Yan-jun and Member, Senior and Tong, Shaocheng and Member, Senior and Chen, C L Philip},
    number = {10},
    pages = {1--10},
    volume = {47}
}

@article{Gao2017BacksteppingSystems,
    title = {{Backstepping design of adaptive neural fault-tolerant control for MIMO nonlinear systems}},
    year = {2017},
    journal = {IEEE Transactions on Neural Networks and Learning Systems},
    author = {Gao, Hui and Song, Yongduan and Wen, Changyun},
    number = {11},
    pages = {2605--2613},
    volume = {28},
    doi = {10.1109/TNNLS.2016.2599009},
    issn = {21622388},
    keywords = {Fault-tolerant control, Filter-based modification, Globally uniformly bounded, Neural networks (NNs)}
}

@article{Ascencio2017BacksteppingApproach,
    title = {{Backstepping PDE Design: A Convex Optimization Approach}},
    year = {2017},
    journal = {IEEE Transactions on Automatic Control},
    author = {Ascencio, Pedro and Astolfi, Alessandro and Parisini, Thomas},
    number = {c},
    pages = {1--16},
    volume = {9286},
    isbn = {9781479978861},
    doi = {10.1109/TAC.2017.2757088},
    issn = {00189286},
    arxivId = {1710.03723},
    keywords = {Backstepping, Backstepping PDE design, Convex Optimization, Convex functions, Distributed Parameter Systems, Hilbert space, Integral equations, Kernel, Mathematical model, Sum-of-Squares, Tools}
}

@article{Engineering2006BasedApproach,
    title = {{Based on Fuzzy-Neural Approach}},
    year = {2006},
    author = {Engineering, Naval Aeronautical},
    pages = {519--523},
    keywords = {adaptive control, backstepping, fuzzy-neural approximator, nonaffine system}
}

@book{Bolotin2009Chaos:Use,
    title = {{Chaos: Concepts, Control and Constructive Use}},
    year = {2009},
    author = {Bolotin, Yurii and Tur, Anatoli and Yanovsky, Vladimir},
    url = {http://link.springer.com/10.1007/978-3-642-00937-2},
    isbn = {978-3-642-00936-5},
    doi = {10.1007/978-3-642-00937-2},
    issn = {1860-0832}
}

@book{Li2016CommunicationsGrids,
    title = {{Communications for Control in Cyber Physical Systems: Theory, Design and Applications in Smart Grids}},
    year = {2016},
    author = {Li, H},
    isbn = {9780128019504}
}

@article{Yi2017CompositeConvergence,
    title = {{Composite backstepping control with finite-time convergence}},
    year = {2017},
    journal = {Optik},
    author = {Yi, Sheng and Wang, Jiang and Li, Bin},
    pages = {260--272},
    volume = {142},
    publisher = {Elsevier GmbH.},
    url = {http://dx.doi.org/10.1016/j.ijleo.2017.05.070},
    doi = {10.1016/j.ijleo.2017.05.070},
    issn = {00304026},
    keywords = {Angle-of-attack tracking, Backstepping, Extended state observer, Finite-time convergent differentiator, Mismatched uncertainty, Missile autopilot}
}

@article{Xian2017ContinuousDisturbance,
    title = {{Continuous Asymptotically Tracking Control for a Class of Nonaffine-in-Input System with Nonvanishing Disturbance}},
    year = {2017},
    journal = {IEEE Transactions on Automatic Control},
    author = {Xian, Bin and Zhang, Yao},
    number = {11},
    pages = {6019--6025},
    volume = {62},
    doi = {10.1109/TAC.2017.2704025},
    issn = {00189286},
    keywords = {Disturbance, nonaffine, robust, tracking}
}

@article{Dai2014ControlSystems,
    title = {{Control of a Class of Nonaffine Nonlinear Systems}},
    year = {2014},
    author = {Dai, Shi-lu and Wang, Cong and Wang, Min},
    number = {1},
    pages = {111--123},
    volume = {25}
}

@article{Yang2008ControlNetworks,
    title = {{Control of nonaffine nonlinear discrete-time systems using reinforcement-learning-based linearly parameterized neural networks}},
    year = {2008},
    journal = {IEEE Transactions on Systems, Man, and Cybernetics, Part B: Cybernetics},
    author = {Yang, Qinmin and Vance, Jonathan Blake and Jagannathan, S.},
    number = {4},
    pages = {994--1001},
    volume = {38},
    isbn = {1941-0492 (Electronic){\textbackslash}r1083-4419 (Linking)},
    doi = {10.1109/TSMCB.2008.926607},
    issn = {10834419},
    pmid = {18632390},
    keywords = {Adaptive critic, Adaptive dynamic programming, Lyapunov stability, Neural network control, Reinforcement learning control}
}

@book{Klapp2016ControlSystems,
    title = {{Control of Self- Organizing Nonlinear Systems}},
    year = {2016},
    author = {Klapp, Sabine H L},
    isbn = {9783319280271}
}

@book{BrecherCyber-PhysicalAnd,
    title = {{Cyber-Physical Systems Cyber-Physical Systems Foundations , Principles and}},
    author = {Brecher, Christian},
    isbn = {9780128038017}
}

@article{Karimi2009DecentralizedSystems,
    title = {{Decentralized Adaptive Control of Large-Scale Affine and Nonaffine Nonlinear Systems}},
    year = {2009},
    journal = {IEEE Transactions on Instrumentation and Measurement},
    author = {Karimi, B. and Menhaj, M.B. and Karimi-Ghartemani, M. and Saboori, I.},
    number = {8},
    pages = {2459--2467},
    volume = {58},
    doi = {10.1109/TIM.2009.2016388},
    issn = {0018-9456},
    keywords = {Adaptive control, decentralized affine and nonaffine nonlinear syste, radial basis neural network (RBNN)}
}

@article{Park2005DirectNetworks.,
    title = {{Direct adaptive controller for nonaffine nonlinear systems using self-structuring neural networks.}},
    year = {2005},
    journal = {IEEE transactions on neural networks},
    author = {Park, Jang-Hyun and Huh, Sung-Hoe and Kim, Seong-Hwan and Seo, Sam-Jun and Park, Gwi-Tae},
    number = {2},
    pages = {414--22},
    volume = {16},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/15787148},
    doi = {10.1109/TNN.2004.841786},
    issn = {1045-9227},
    pmid = {15787148},
    keywords = {Adaptation, Neural Networks (Computer), Nonlinear Dynamics, Physiological}
}

@article{Chen2013DirectObserver.,
    title = {{Direct Adaptive Neural Control for a Class of Uncertain Nonaffine Nonlinear Systems Based on Disturbance Observer.}},
    year = {2013},
    journal = {IEEE transactions on cybernetics},
    author = {Chen, Mou and Ge, Shuzhi Sam},
    number = {4},
    month = {8},
    pages = {1213--25},
    volume = {43},
    url = {http://ieeexplore.ieee.org/document/6374742/ http://www.ncbi.nlm.nih.gov/pubmed/26502431},
    doi = {10.1109/TSMCB.2012.2226577},
    issn = {2168-2275},
    pmid = {26502431},
    keywords = {Adaptive control, Disturbance observer, Input saturation, Neural networks (NNs), Nonaffine nonlinear system}
}

@article{Behera2016DiscreteFeedback,
    title = {{Discrete event-triggered sliding mode control with fast output sampling feedback}},
    year = {2016},
    journal = {Proceedings of IEEE International Workshop on Variable Structure Systems},
    author = {Behera, Abhisek K. and Bandyopadhyay, Bijnan and Reger, Johann},
    pages = {148--153},
    volume = {2016-July},
    isbn = {9781467397889},
    doi = {10.1109/VSS.2016.7506907},
    issn = {21654824},
    keywords = {Event-triggered control, discrete-time sliding mode control, multirate output feedback}
}

@article{Guan2012DynamicDelays,
    title = {{Dynamic surface control for a class of state-constrained non-linear systems with uncertain time delays}},
    year = {2012},
    journal = {IET Control Theory {\&} Applications},
    author = {Guan, X.-P. and Wu, X.-J. and Wu, X.-L. and Luo, X.-Y.},
    number = {12},
    pages = {1948--1957},
    volume = {6},
    url = {http://digital-library.theiet.org/content/journals/10.1049/iet-cta.2011.0543},
    doi = {10.1049/iet-cta.2011.0543},
    issn = {1751-8644}
}

@article{Li2017Event-BasedSystems,
    title = {{Event-Based Adaptive {\{}NN{\}} Tracking Control of Nonlinear Discrete-Time Systems}},
    year = {2017},
    journal = {{\{}IEEE{\}} Transactions on Neural Networks and Learning Systems},
    author = {Li, Yuan-Xin and Yang, Guang-Hong},
    pages = {1--11},
    url = {https://doi.org/10.1109%2Ftnnls.2017.2765683},
    doi = {10.1109/tnnls.2017.2765683}
}

@article{Eqtami2010Event-triggeredSystems,
    title = {{Event-triggered Control for Discrete-Time Systems}},
    year = {2010},
    journal = {2010 American Control Conference},
    author = {Eqtami, Alina and Dimarogonas, Dimos V and Kyriakopoulos, Kostas J},
    pages = {4719--4724},
    url = {http://apps.webofknowledge.com/full_record.do?product=UA&search_mode=GeneralSearch&qid=6&SID=W1odEfKka67fCPtCVHO&page=1&doc=8&cacheurlFromRightClick=no},
    isbn = {978-1-4244-7427-1},
    doi = {10.1109/ACC.2010.5531089},
    issn = {0743-1619},
    keywords = {NONLINEAR-SYSTEMS, STABILITY}
}

@book{BeheraEvent-TriggeredControl,
    title = {{Event-Triggered Sliding Mode Control}},
    author = {Behera, Abhisek K},
    isbn = {9783319742182}
}

@article{Behera2016Event-triggeredSystems,
    title = {{Event-triggered sliding mode control for a class of nonlinear systems}},
    year = {2016},
    journal = {International Journal of Control},
    author = {Behera, Abhisek K. and Bandyopadhyay, Bijnan},
    number = {9},
    pages = {1916--1931},
    volume = {89},
    publisher = {Taylor {\&} Francis},
    url = {http://dx.doi.org/10.1080/00207179.2016.1142617},
    doi = {10.1080/00207179.2016.1142617},
    issn = {13665820},
    keywords = {Nonlinear systems, event-triggered control, robust stabilisation, sliding mode control}
}

@book{Li2016FaultSystems,
    title = {{Fault Detection and Fault-Tolerant Control for Nonlinear Systems}},
    year = {2016},
    author = {Li, Linlin},
    url = {http://link.springer.com/10.1007/978-3-658-13020-6},
    isbn = {978-3-658-13019-0},
    doi = {10.1007/978-3-658-13020-6}
}

@book{Zolghadri2014FaultVehicles,
    title = {{Fault Diagnosis and Fault-Tolerant Control and Guidance for Aerospace Vehicles}},
    year = {2014},
    author = {Zolghadri, Ali and Henry, David and Cieslak, Jérôme and Efimov, Denis and Goupil, Philippe},
    url = {http://link.springer.com/10.1007/978-1-4471-5313-9},
    isbn = {978-1-4471-5312-2},
    doi = {10.1007/978-1-4471-5313-9}
}

@book{Shen2017FaultApproach,
    title = {{Fault Diagnosis and Fault-Tolerant Control Based on Adaptive Control Approach}},
    year = {2017},
    author = {Shen, Qikun and Jiang, Bin and Shi, Peng},
    volume = {91},
    url = {http://link.springer.com/10.1007/978-3-319-52530-3},
    isbn = {978-3-319-52529-7},
    doi = {10.1007/978-3-319-52530-3}
}

@article{Deng2008Feedback-linearization-basedSystems,
    title = {{Feedback-linearization-based neural adaptive control for unknown nonaffine nonlinear discrete-time systems}},
    year = {2008},
    journal = {IEEE Transactions on Neural Networks},
    author = {Deng, Hua and Li, Han Xiong and Wu, Yi Hu},
    number = {9},
    pages = {1615--1625},
    volume = {19},
    doi = {10.1109/TNN.2008.2000804},
    issn = {10459227},
    pmid = {18779092},
    keywords = {Feedback linearization, Neural networks, Nonaffine nonlinear discrete-time systems, Nonlinear adaptive control}
}

@article{Efe2011FractionalSurvey,
    title = {{Fractional Order Systems in Industrial Automation — A Survey}},
    year = {2011},
    journal = {IEEE Transactions on Industrial Informatics},
    author = {Efe, Mehmet Önder and Member, Senior},
    number = {4},
    pages = {582--591},
    volume = {7},
    isbn = {1551-3203},
    doi = {Doi 10.1109/Tii.2011.2166775},
    issn = {1551-3203}
}

@article{Tong2015FuzzyConstrained,
    title = {{Fuzzy Adaptive Output Feedback Control of MIMO Nonlinear Systems with Partial Tracking Errors Constrained}},
    year = {2015},
    journal = {IEEE Transactions on Fuzzy Systems},
    author = {Tong, Shaocheng and Sui, Shuai and Li, Yongming},
    number = {4},
    pages = {729--742},
    volume = {23},
    isbn = {1063-6706},
    doi = {10.1109/TFUZZ.2014.2327987},
    issn = {10636706},
    keywords = {Adaptive fuzzy control, partial state tracking errors constrained, prescribed performance function, stability analysis, state observer design, uncertain MIMO nonlinear systems}
}

@article{Khalil2017High-GainMotors,
    title = {{High-Gain Observers in Feedback Control: Application to Permanent Magnet Synchronous Motors}},
    year = {2017},
    journal = {IEEE Control Systems},
    author = {Khalil, Hassan K.},
    number = {3},
    pages = {25--41},
    volume = {37},
    isbn = {9781424447060},
    doi = {10.1109/MCS.2017.2674438},
    issn = {1066033X},
    pmid = {18795146},
    arxivId = {arXiv:1505.02595v1}
}

@article{Dai2012IdentificationNetworks,
    title = {{Identification and learning control of ocean surface ship using neural networks}},
    year = {2012},
    journal = {IEEE Transactions on Industrial Informatics},
    author = {Dai, Shi Lu and Wang, Cong and Luo, Fei},
    number = {4},
    pages = {801--810},
    volume = {8},
    isbn = {1551-3203},
    doi = {10.1109/TII.2012.2205584},
    issn = {15513203},
    keywords = {Adaptive neural network (NN) control, learning, persistent excitation (PE) condition, ship control, uncertain dynamics}
}

@article{Wei2015InfiniteOf,
    title = {{Infinite Horizon Self-Learning Optimal Control of}},
    year = {2015},
    author = {Wei, Qinglai and Liu, Derong and Yang, Xiong},
    number = {4},
    pages = {866--879},
    volume = {26}
}

@article{Zhang2013IntegralUncertainty,
    title = {{Integral Terminal Sliding Mode Control for a Class of Nonaffine Nonlinear Systems with Uncertainty}},
    year = {2013},
    author = {Zhang, Qiang and Yu, Hongliang and Wang, Xiaohong},
    volume = {2013},
    doi = {10.1155/2013/636494},
    issn = {15635147}
}

@book{DesignIntelligentSimulation,
    title = {{Intelligent Control Design and M at L ab Simulation}},
    author = {Design, Intelligent Control},
    isbn = {9789811052620}
}

@book{Dr-IngDierkSchroder2000IntelligentDierk,
    title = {{Intelligent Observer and Control Design for Nonlinear Systems Library of Congress Cataloging-in-Publication Data applied for Die Deutsche Bibliothek -Cip-Einheitsaufnahme Intelligent ob server and control design for nonlinear systems! Dierk}},
    year = {2000},
    booktitle = {Hong Kong; London; Milan; Paris; Singapore},
    author = {Dr-Ing Dierk Schr{\"{o}}der, Dr-Ing and Dr-Ing Dierk Schr{\"{o}}der Dr-Ing UlrichLenz Dipl-Ing Michael Beuschel Dipl-Ing FranzD Hangl Dr-Ing ThomasFrenz Dr-Ing Dieter Strobl Dr-Ing Stephan Straub Dr-Ing Kurt Fischle Dipl-IngMartinRau Dipl-Ing Anne Angermann, Dr-Ing},
    url = {http://dlx.b-ok.org/genesis/939000/2b06948dca36e2dcaeb854465ad7a6ed/_as/[Dierk_Schröder__(auth.),__Prof._Dr.-Ing._Dr.-Ing(b-ok.org).pdf},
    isbn = {978-3-662-04117-8},
    doi = {10.1007/978-3-662-04117-8}
}

@book{EditionIntroductionScientists,
    title = {{Introduction To Probability and Statistics for Engineers and Scientists}},
    author = {Edition, Third},
    url = {http://www.r-5.org/files/books/computers/algo-list/statistics/Sheldon_Ross-Introduction_to_Probability_and_Statistics-EN.pdf},
    isbn = {0125980574}
}

@article{Choe2015L1Systems,
    title = {{L1 Adaptive Control for a Class of Uncertain Nonaffine-in-Control Nonlinear Systems}},
    year = {2015},
    journal = {IEEE Transactions on Automatic Control},
    author = {Choe, Ronald and Xargay, Enric and Hovakimyan, Naira},
    number = {3},
    pages = {1--1},
    volume = {61},
    url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=7140742},
    doi = {10.1109/TAC.2015.2451491},
    issn = {0018-9286}
}

@article{LyapunovLecture2,
    title = {{Lecture 2}},
    author = {Lyapunov, Unlike},
    pages = {13--25}
}

@article{BelavkinLectureRule,
    title = {{Lecture 7 : Ito differentiation rule}},
    author = {Belavkin, Roman V},
    pages = {1--5},
    url = {http://www.eis.mdx.ac.uk/staffpages/rvb/teaching/MSO4112/hand07.pdf}
}

@article{Zhao2007LocallySystems,
    title = {{Locally weighted online approximation-based control for nonaffine systems}},
    year = {2007},
    journal = {IEEE Transactions on Neural Networks},
    author = {Zhao, Yuanyuan and Farrell, Jay A.},
    number = {6},
    pages = {1709--1724},
    volume = {18},
    doi = {10.1109/TNN.2007.895908},
    issn = {10459227},
    keywords = {Adaptive approximation-based control, Adaptive nonlinear control, Locally weighted learning (LWL), Nonaffine systems, Receptive field weighted regression}
}

@article{Aguila-Camacho2014LyapunovSystems,
    title = {{Lyapunov functions for fractional order systems}},
    year = {2014},
    journal = {Communications in Nonlinear Science and Numerical Simulation},
    author = {Aguila-Camacho, Norelys and Duarte-Mermoud, Manuel A. and Gallegos, Javier A.},
    number = {9},
    pages = {2951--2957},
    volume = {19},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.cnsns.2014.01.022},
    isbn = {1007-5704},
    doi = {10.1016/j.cnsns.2014.01.022},
    issn = {10075704},
    keywords = {Fractional calculus, Fractional-order Lyapunov direct method, Stability of fractional order systems}
}

@article{Shpitser2017ModelingDecomposition,
    title = {{Modeling Interference Via Symmetric Treatment Decomposition}},
    year = {2017},
    author = {Shpitser, Ilya and Tchetgen, Eric Tchetgen and Andrews, Ryan},
    number = {April 2014},
    pages = {1844--1861},
    url = {http://arxiv.org/abs/1709.01050},
    isbn = {9120256922},
    doi = {10.1002/rnc},
    arxivId = {1709.01050},
    keywords = {10.1002/rnc.3181 and adaptive control, Lyapunov method, MIMO, NN, adaptive control, discrete-time, feedback control, lyapunov method, mimo, nn, nonaffine system, online learning}
}

@book{Manfredi2017MultilayerSystems,
    title = {{Multilayer Control of Networked Cyber-Physical Systems}},
    year = {2017},
    author = {Manfredi, Sabato},
    url = {http://link.springer.com/10.1007/978-3-319-41646-5},
    isbn = {978-3-319-41645-8},
    doi = {10.1007/978-3-319-41646-5}
}

@book{MorariNeuralNonlinear,
    title = {{Neural Network-Based State Estimation of Nonlinear}},
    author = {Morari, M},
    isbn = {9781441914378}
}

@article{Ge2003Neural-NetworkAnd,
    title = {{Neural-Network Control of Nonaffine Nonlinear System With Zero Dynamics by State and}},
    year = {2003},
    author = {Ge, Shuzhi Sam and Member, Senior and Zhang, Jin},
    number = {4},
    pages = {900--918},
    volume = {14}
}

@article{2018NoTitle,
    title = {{No Title}},
    year = {2018},
    pages = {5772018}
}

@book{NoTitle,
    title = {{No Title}},
    isbn = {9781482263169}
}

@book{vandeWouw1996NonlinearSystems,
    title = {{Nonlinear Systems}},
    year = {1996},
    author = {van de Wouw, Nathan and Lefeber, Erjen and Lopez Arteaga, Ines},
    pages = {1 - 748},
    isbn = {0132280248},
    doi = {10.1007/978-1-4757-3108-8},
    issn = {0949-1775},
    pmid = {1617627}
}

@article{Leu2005Observer-basedSystems,
    title = {{Observer-based direct adaptive fuzzy-neural control for nonaffine nonlinear systems}},
    year = {2005},
    journal = {IEEE Transactions on Neural Networks},
    author = {Leu, Yih Guang and Wang, Wei Yen and Lee, Tsu Tian},
    number = {4},
    pages = {853--861},
    volume = {16},
    isbn = {1045-9227},
    doi = {10.1109/TNN.2005.849824},
    issn = {10459227},
    pmid = {16121727},
    keywords = {Direct adaptive control, Fuzzy-neural control, Nonaffine nonlinear systems, Output feedback control}
}

@article{Laws2011Observer-BasedUsing,
    title = {{Observer-Based T – S Fuzzy Control for a Class of General Nonaffine Nonlinear Systems Using}},
    year = {2011},
    author = {Laws, Generalized Projection-update and Wang, Wei-yen and Member, Senior and Chien, Yi-hsing and Lee, Tsu-tian and Statement, A Problem},
    number = {3},
    pages = {493--504},
    volume = {19}
}

@book{Topics2012OPTIMALMATLAB,
    title = {{OPTIMAL and ROBUST CONTROL Advanced Topics with MATLAB}},
    year = {2012},
    booktitle = {Taylor {\&} Francis Group},
    author = {Topics, Advanced},
    pages = {1--250},
    isbn = {9781466503151}
}

@book{Sarangapani2016OptimalMATLAB,
    title = {{Optimal Networked Control Systems with MATLAB}},
    year = {2016},
    author = {Sarangapani, Jagannathan and Xu, Hao},
    pages = {1--5},
    isbn = {9781482235265}
}

@article{Deng1999Output-feedbackStabilization,
    title = {{Output-feedback stochastic nonlinear stabilization}},
    year = {1999},
    journal = {IEEE Transactions on Automatic Control},
    author = {Deng, Hua and Krsti{\'{c}}, Miroslav},
    number = {2},
    pages = {328--333},
    volume = {44},
    isbn = {0-7803-4187-2},
    doi = {10.1109/9.746260},
    issn = {00189286},
    keywords = {Backstepping, Control lyapunov functions, Inverse optimality, Stochastic nonlinear output-feedback systems, Stochastic stabilization}
}

@misc{Philip2003.pdf,
    title = {{Philip E. Protter-Stochastic Integration and Differential Equations -Springer (2003).pdf}}
}

@article{Knill2009ProbabilityApplications,
    title = {{Probability Theory and Stochastic Processes with Applications}},
    year = {2009},
    author = {Knill, Oliver},
    pages = {373},
    url = {www.math.harvard.edu/~knill/teaching/math144_1994/probability.pdf},
    isbn = {978-8189938406},
    doi = {10.1007/978-3-662-12616-5{\_}2}
}

@book{Bishop1995RadialFunctions,
    title = {{Radial Basis Functions}},
    year = {1995},
    booktitle = {Neural Networks for Pattern Recognition},
    author = {Bishop, Christopher M.},
    pages = {1--374},
    isbn = {9780511543241},
    doi = {10.1017/CBO9780511543241},
    issn = {1098-6596},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {Neural adaptive control, manipulator, radial basis function}
}

@book{Wang2013ResourceConstraints,
    title = {{Resource Scheduling of Cloud with QoS Constraints}},
    year = {2013},
    booktitle = {Advances in Neural Networks - ISNN 2013},
    author = {Wang, Yan and Wang, Jinkuan and Wang, Cuirong and Song, Xin},
    number = {July},
    pages = {351--358},
    isbn = {9783540342915},
    doi = {10.1007/3-540-68339-9{\_}34},
    issn = {0302-9743},
    pmid = {4520227},
    arxivId = {9780201398298}
}

@book{Corke2011RoboticsControl,
    title = {{Robotics, Vision and Control}},
    year = {2011},
    author = {Corke, Peter},
    volume = {73},
    url = {http://link.springer.com/10.1007/978-3-642-20144-8},
    isbn = {978-3-642-20143-1},
    doi = {10.1007/978-3-642-20144-8},
    issn = {00219606},
    pmid = {19105594},
    arxivId = {arXiv:cond-mat/0509398v1},
    archivePrefix = {arXiv},
    eprint = {0509398v1},
    primaryClass = {cond-mat}
}

@article{Adetona2004RobustChanges,
    title = {{Robust adaptive control of nonaffine nonlinear plants with small input signal changes}},
    year = {2004},
    journal = {IEEE Transactions on Neural Networks},
    author = {Adetona, O. and Sathananthan, S. and Keel, L. H.},
    number = {2},
    pages = {408--416},
    volume = {15},
    doi = {10.1109/TNN.2004.824423},
    issn = {10459227},
    pmid = {15384533},
    keywords = {Adaptive control, Approximate models, Asymptotic tracking, Input-output models, Neural networks, Nonaffine nonlinear control}
}

@article{Fan2003RobustPhilosophy,
    title = {{Robust Adaptive Control of Uncertain Nonlinear Systems By for the Degree of Doctor of Philosophy}},
    year = {2003},
    author = {Fan, Hong}
}

@article{Wen2011RobustDisturbance,
    title = {{Robust adaptive control of uncertain nonlinear systems in the presence of input saturation and external disturbance}},
    year = {2011},
    journal = {IEEE Transactions on Automatic Control},
    author = {Wen, Changyun and Zhou, Jing and Liu, Zhitao and Su, Hongye},
    number = {7},
    pages = {1672--1678},
    volume = {56},
    isbn = {0018-9286 VO - 56},
    doi = {10.1109/TAC.2011.2122730},
    issn = {00189286},
    keywords = {Adaptive control, backstepping, global stability, nonlinear systems, saturation}
}

@article{Shi2017RobustSystems,
    title = {{Robust adaptive neural control for a class of non-affine nonlinear systems}},
    year = {2017},
    journal = {Neurocomputing},
    author = {Shi, Chao and Dong, Xinmin and Xue, Jianping and Chen, Yong and Zhi, Jianhui},
    pages = {118--128},
    volume = {223},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.neucom.2016.10.029},
    doi = {10.1016/j.neucom.2016.10.029},
    issn = {18728286},
    keywords = {Adaptive control, Invariant set, Neural network, Non-affine nonlinear systems}
}

@article{Ge2002RobustSystems,
    title = {{Robust adaptive nn control of a class of semi-strict feedback nonlinear systems}},
    year = {2002},
    journal = {IFAC Proceedings Volumes (IFAC-PapersOnline)},
    author = {Ge, S. S. and Wang, J. and Lee, T. H.},
    number = {1},
    pages = {433--438},
    volume = {35},
    doi = {10.1109/TNN.2002.804306},
    issn = {14746670},
    pmid = {18244537},
    keywords = {Neural networks, Robust adaptive control, Semi-strict feedback nonlinear systems}
}

@article{Chen2013RobustVessels,
    title = {{Robust adaptive position mooring control for marine vessels}},
    year = {2013},
    journal = {IEEE Transactions on Control Systems Technology},
    author = {Chen, Mou and Ge, Shuzhi Sam and How, Bernard Voon Ee and Choo, Yoo Sang},
    number = {2},
    pages = {395--409},
    volume = {21},
    doi = {10.1109/TCST.2012.2183676},
    issn = {10636536},
    keywords = {Backstepping control, control allocation, mooring systems, nonlinear systems, robust adaptive control}
}

@article{Ge2003RobustCoefficients,
    title = {{Robust adaptive tracking for time-varying uncertain nonlinear systems with unknown control coefficients}},
    year = {2003},
    journal = {Automatic Control, IEEE Transactions on},
    author = {Ge, Shuzhi Sam and Wang, Jing},
    number = {8},
    pages = {1463--1469},
    volume = {48},
    issn = {0018-9286}
}

@article{Chen2015RobustObserver,
    title = {{Robust Constrained Control for MIMO Nonlinear Systems Based on Disturbance Observer}},
    year = {2015},
    journal = {Automatic Control, IEEE Transactions on},
    author = {Chen, Mou and Shi, Peng and Lim, Cheng-chew and Member, Senior},
    number = {12},
    pages = {3281--3286},
    volume = {60},
    isbn = {0018-9286},
    doi = {10.1109/TAC.2015.2450891},
    issn = {00189286}
}

@article{Ren2015RobustEstimator,
    title = {{Robust Control for a Class of Nonaffine Nonlinear Systems Based on the Uncertainty and Disturbance Estimator}},
    year = {2015},
    journal = {IEEE Transactions on Industrial Electronics},
    author = {Ren, Beibei and Zhong, Qing Chang and Chen, Jinhao},
    number = {9},
    pages = {5881--5888},
    volume = {62},
    isbn = {0278-0046},
    doi = {10.1109/TIE.2015.2421884},
    issn = {02780046},
    keywords = {Disturbance, nonaffine systems, nonlinear systems, robust control, uncertainty, uncertainty and disturbance estimator (UDE)}
}

@article{Levant1998RobustTechnique,
    title = {{Robust Exact Differentiation via Sliding Mode Technique}},
    year = {1998},
    journal = {Automatica},
    author = {Levant, Arie},
    number = {3},
    pages = {379--384},
    volume = {34},
    isbn = {9727623131},
    doi = {10.1016/S0005-1098(97)00209-4},
    issn = {00051098},
    keywords = {Differentiators, Measurement noise, Nonlinear control, Robustness, Sliding mode}
}

@article{Lee2004RobustEstimation,
    title = {{Robust Extended Kalman Filtering via Krein Space Estimation}},
    year = {2004},
    journal = {IEICE Transactions on Fundamentals of Electronics, Communications and Computer Sciences},
    author = {Lee, Tae Hoon and Ra, Won Sang and Jin, Seung Hee and Yoon, Tae Sung and Park, Jin Bae},
    number = {1},
    pages = {243--250},
    volume = {E87-A},
    isbn = {9781479902248},
    doi = {10.1049/ip-cta},
    issn = {09168508},
    keywords = {Discrete-time nonlinear system, Extended Kalman filter, Krein space, Parameter uncertainty, Robust Kalman filter}
}

@article{Bounemeur2014RobustDirections,
    title = {{Robust indirect adaptive fuzzy control using Nussbaum gain for a class of SISO nonlinear systems with unknown directions}},
    year = {2014},
    journal = {STA 2014 - 15th International Conference on Sciences and Techniques of Automatic Control and Computer Engineering},
    author = {Bounemeur, A. and Chemachema, M. and Essounbouli, N.},
    pages = {748--754},
    isbn = {9781479959075},
    doi = {10.1109/STA.2014.7086763},
    keywords = {Lyapunov stability, adaptive fuzzy control, nonlinear systems}
}

@book{Zhang2016RobustMATLAB,
    title = {{Robust Observer Based Fault Diagnosis for Nonlinear Systems Using MATLAB}},
    year = {2016},
    author = {Zhang, Jian and Kumar, Akshya and Kiong, Sing},
    pages = {223},
    isbn = {9783319323237},
    doi = {10.1007/978-3-319-32324-4}
}

@article{Xi2017RobustOf,
    title = {{Robust Sliding Mode Control of}},
    year = {2017},
    journal = {Mechanical Engineering},
    author = {Xi, Mechanical Engineering},
    number = {2},
    pages = {430--437},
    volume = {64},
    isbn = {8145476372},
    keywords = {energy control, nonlinear, wind}
}

@book{Shtessel2014SlidingObservation,
    title = {{Sliding Mode Control and Observation}},
    year = {2014},
    booktitle = {Nota},
    author = {Shtessel, Yuri B. and Edwards, Christopher and Fridman, Leonid M. and Levant, Arie},
    pages = {1--43},
    url = {https://books.google.co.uk/books?id=jYQ_AAAAQBAJ%5Cnhttp://link.springer.com/10.1007/978-0-8176-4893-0},
    isbn = {978-0-8176-4892-3},
    doi = {10.1007/978-0-8176-4893-0},
    issn = {15715078}
}

@article{Ren2018SlidingNonlinearities,
    title = {{Sliding mode control for a class of positive systems with Lipschitz nonlinearities}},
    year = {2018},
    journal = {IEEE Access},
    author = {Ren, Chengcheng and He, Shuping},
    pages = {1--1},
    volume = {6},
    publisher = {IEEE},
    url = {https://ieeexplore.ieee.org/document/8453786/},
    doi = {10.1109/ACCESS.2018.2868344},
    issn = {2169-3536}
}

@article{Han2013SlidingManipulator,
    title = {{Sliding Mode Control for Guaranteed Tracking Performance of Robot Manipulator}},
    year = {2013},
    author = {Han, Seong Ik and Cheong, Jeong Yun and Lee, Jang Myung},
    volume = {2013}
}

@article{SCOPUS2017SourcePublication,
    title = {{Source Publication}},
    year = {2017},
    author = {{SCOPUS}},
    number = {July},
    issn = {1839-2571}
}

@book{Lin2015StabilitySystems,
    title = {{Stability Analysis of Nonlinear Systems}},
    year = {2015},
    author = {Lin, Zongli},
    pages = {40},
    volume = {1},
    isbn = {9783319271996},
    doi = {10.1007/978-3-319-27200-9}
}

@book{Breda2015StabilityMATLAB,
    title = {{Stability of Linear Delay Differential Equations: A Numerical Approach with MATLAB}},
    year = {2015},
    author = {Breda, D and Maset, S and Vermiglio, R},
    isbn = {9781493921072},
    issn = {21926794}
}

@article{Moulay2005StabilizationSystems,
    title = {{Stabilization of nonaffine systems: A constructive method for polynomial systems}},
    year = {2005},
    journal = {IEEE Transactions on Automatic Control},
    author = {Moulay, Emmanuel and Perruquetti, Wilfrid},
    number = {4},
    pages = {520--526},
    volume = {50},
    doi = {10.1109/TAC.2005.844899},
    issn = {00189286},
    keywords = {Control Lyapunov function, Nonaffine systems, Polynomial systems, Stabilization}
}

@article{Deng1998StabilizationCovariance,
    title = {{Stabilization of stochastic nonlinear systems driven by noise of unknown covariance}},
    year = {1998},
    journal = {Proceedings of the American Control Conference},
    author = {Deng, Hua and Krsti??, Miroslav},
    pages = {269--278},
    volume = {1},
    isbn = {0780345304},
    doi = {10.1109/ACC.1998.694673},
    issn = {07431619},
    keywords = {adaptive stabilization, noise-to-state stabilization, output-feedback stabilization}
}

@article{Deng1998StabilizationCovarianceb,
    title = {{Stabilization of stochastic nonlinear systems driven by noise of unknown covariance}},
    year = {1998},
    journal = {Proceedings of the American Control Conference},
    author = {Deng, Hua and Krsti??, Miroslav},
    number = {8},
    pages = {269--278},
    volume = {1},
    isbn = {0780345304},
    doi = {10.1109/ACC.1998.694673},
    issn = {07431619}
}

@article{Herzog2013StochasticEquations,
    title = {{Stochastic Differential Equations}},
    year = {2013},
    author = {Herzog, Florian},
    pages = {1--64},
    url = {https://www.ethz.ch/content/dam/ethz/special-interest/mavt/dynamic-systems-n-control/idsc-dam/Lectures/Stochastic-Systems/SDE.pdf}
}

@article{Deng1997StochasticDesign,
    title = {{Stochastic nonlinear stabilization - I: A backstepping design}},
    year = {1997},
    journal = {Systems and Control Letters},
    author = {Deng, Hua and Krsti{\'{c}}, Miroslav},
    number = {3},
    pages = {143--150},
    volume = {32},
    doi = {10.1016/S0167-6911(97)00068-6},
    issn = {01676911},
    keywords = {Backstepping, Stochastic nonlinear systems}
}

@article{Deng1997StochasticOptimality,
    title = {{Stochastic nonlinear stabilization - II: Inverse optimality}},
    year = {1997},
    journal = {Systems and Control Letters},
    author = {Deng, Hua and Krsti{\'{c}}, Miroslav},
    number = {3},
    pages = {151--159},
    volume = {32},
    doi = {10.1016/S0167-6911(97)00067-4},
    issn = {01676911},
    keywords = {Backstepping, Control Lyapunov functions, Stochastic nonlinear systems}
}

@book{Khasminskii2011StochasticProbability,
    title = {{Stochastic Stability of Differential Equations (Stochastic Modelling and Applied Probability)}},
    year = {2011},
    author = {Khasminskii, Rafail},
    pages = {400},
    url = {http://www.amazon.com/Stochastic-Stability-Differential-Equations-Probability/dp/3642232795},
    isbn = {3642232795},
    doi = {10.1007/978-3-642-23280-0}
}

@article{Han2014SurfaceSystem,
    title = {{Surface Control for a Strict Feedback Nonlinear Dynamic System}},
    year = {2014},
    author = {Han, Seong I and Lee, Jang M and Member, Senior},
    number = {5},
    pages = {1049--1061},
    volume = {22},
    isbn = {8251514169},
    doi = {10.1109/TIE.2014.2316263}
}

@article{Anta2010ToSystems,
    title = {{To sample or not to sample: Self-triggered control for nonlinear systems}},
    year = {2010},
    journal = {IEEE Transactions on Automatic Control},
    author = {Anta, Adolfo and Tabuada, Paulo},
    number = {9},
    pages = {2030--2042},
    volume = {55},
    isbn = {0018-9286},
    doi = {10.1109/TAC.2010.2042980},
    issn = {00189286},
    arxivId = {0806.0709},
    keywords = {Networked control, Nonlinear control, Real-time control systems, Self-triggered control}
}

@article{Song2016TrackingApproach,
    title = {{Tracking control for a class of unknown nonsquare MIMO nonaffine systems: A deep-rooted information based robust adaptive approach}},
    year = {2016},
    journal = {IEEE Transactions on Automatic Control},
    author = {Song, Yongduan and Huang, Xiucai and Wen, Changyun},
    number = {10},
    pages = {3227--3233},
    volume = {61},
    doi = {10.1109/TAC.2015.2508741},
    issn = {00189286},
    keywords = {Deep-rooted information, Nonsquare nonaffine systems, Robust adaptive control, Virtual parameter}
}

@article{Dong2012TrackingApproach,
    title = {{Tracking control for nonaffine systems: A self-organizing approximation approach}},
    year = {2012},
    journal = {IEEE Transactions on Neural Networks and Learning Systems},
    author = {Dong, Wenjie and Zhao, Yuanyuan and Chen, Yiming and Farrell, Jay A.},
    number = {2},
    pages = {223--235},
    volume = {23},
    isbn = {9781424420797},
    doi = {10.1109/TNNLS.2011.2178509},
    issn = {2162237X},
    pmid = {24808502},
    keywords = {Adaptive nonlinear control, locally weighted learning, nonaffine systems, self-organizing approximation}
}

@article{Tu2012TutorialControl,
    title = {{Tutorial Session : Event-triggered and Self-triggered Control Event-triggered and self-triggered control}},
    year = {2012},
    author = {Tu, W P M H Heemels and Kth, K H Johansson and Tabuada, Paulo}
}

@book{deCursi2015UncertaintyMatlab,
    title = {{Uncertainty Quantification and Stochastic Modeling with Matlab{\textregistered}}},
    year = {2015},
    booktitle = {Uncertainty Quantification and Stochastic Modeling with Matlab{\textregistered}},
    author = {de Cursi, Souza and Sampaio, Rubens},
    pages = {1--442},
    isbn = {9780081004715},
    doi = {10.1016/C2014-0-04713-2},
    issn = {1548-7660}
}

@book{Gao2017UniversalSystems,
    title = {{Universal Fuzzy Controllers for Non-affine Nonlinear Systems}},
    year = {2017},
    author = {Gao, Qing},
    pages = {142},
    isbn = {978-981-10-1974-6},
    doi = {10.1007/978-981-10-1974-6 ISSN}
}

@article{Gao2014UniversalSystems,
    title = {{Universal Fuzzy Models and Universal Fuzzy Controllers for Discrete-Time Nonlinear Systems}},
    year = {2014},
    journal = {IEEE Transactions on Cybernetics},
    author = {Gao, Q. and Feng, G. and Dong, D. and Liu, L.},
    number = {2},
    pages = {328--341},
    volume = {21},
    doi = {10.1109/TCYB.2014.2338312},
    issn = {21682267}
}

@book{Blondel2004UnsolvedTheory,
    title = {{Unsolved problems in mathematical systems and control theory}},
    year = {2004},
    booktitle = {Control},
    author = {Blondel, V},
    url = {http://books.google.com/books?hl=en&amp;lr=&amp;id=-OwmYdZySwAC&amp;oi=fnd&amp;pg=PR13&amp;dq=Unsolved+Problems+in+Mathematical+Systems+and+Control+Theory&amp;ots=7_ILmT9W-N&amp;sig=ZiDfGJ1TZAQY0RLjsy1FXRwXa7s},
    isbn = {0691117489},
    doi = {10.1109/TAC.2005.846593},
    issn = {15582523}
}

@book{Yan2016VariableSystems,
    title = {{Variable Structure Control of Complex Systems}},
    year = {2016},
    author = {Yan, Xing-gang and Spurgeon, Sarah K and Edwards, Christopher},
    isbn = {9783319489612}
}

@book{HablyStudiesPublis.pdf,
    title = {{[Studies in Systems, Decision and Control 137] Andr{\'{e}}s Ovalle,Ahmad Hably,Seddik Bacha (auth.) - Grid Optimal Integration of Electric Vehicles{\_} Examples with Matlab Implementation (2018, Springer International Publis.pdf}},
    author = {Hably, Ahmad},
    isbn = {9783319731766}
}
